Predictable Sharing of Last-level Cache Partitions for Multi-core Safety-critical Systems

Last-level cache (LLC) partitioning is a technique to provide temporal isolation and low worst-case latency (WCL) bounds when cores access the shared LLC in multicore safety-critical systems. A typical approach to cache partitioning involves allocating a separate partition to a distinct core. A central criticism of this approach is its poor utilization of cache storage. Today's trend of integrating a larger number of cores exacerbates this issue such that we are forced to consider shared LLC partitions for effective deployments. This work presents an approach to share LLC partitions among multiple cores while being able to provide low WCL bounds.

==> conclusion.tex <==
\section{Conclusion and Future Work}
We leave the investigation of memory consistency model as future work.

==> mechanism.tex <==

\section{Scalable, Predictable and Coherent Data Sharing Mechanism}

==> motivation.tex <==

\section{Motivation}
